Slater Transition in the Pyrochlore Cd2Os2O7

Cd2Os2O7 crystallizes in the pyrochlore structure and undergoes a metal-insulator transition (MIT) near 226 K. We have characterized the MIT in Cd2Os2O7 using X-ray diffraction, resistivity at ambient and high pressure, specific heat, magnetization, thermopower, Hall coefficient, and thermal conductivity. Both single crystals and polycrystalline material were examined. The MIT is accompanied by no change in crystal symmetry and a change in unit cell volume of less than 0.05%. The resistivity shows little temperature dependence above 226 K, but increases by 3 orders of magnitude as the sample is cooled to 4 K. The specific heat anomaly resembles a mean-field transition and shows no hysteresis or latent heat. Cd2Os2O7 orders magnetically at the MIT. The magnetization data is consistent with antiferromagnetic order, with a small parasitic ferromagnetic component. The Hall and Seebeck coefficients are consistent with a semiconducting gap opening at the Fermi energy at the MIT. We have also performed electronic structure calculations on Cd2Os2O7. These calculations indicate that Cd2Os2O7 is metallic, with a sharp peak in the density of states at the Fermi energy. We intepret the data in terms of a Slater transition. In this scenario, the MIT is produced by a doubling of the unit cell due to the establishment of antiferromagnetic order. A Slater transition-unlike a Mott transition-is predicted to be continuous, with a semiconducting energy gap opening much like a BCS gap as the material is cooled below $T_{MIT}$.

==> cdosbib.tex <==
@ARTICLE{Sleight66,
   author = "A.W. Sleight and J.L. Gillson",
   year = "1966",
   journal = "Solid State Comm.",
   volume = "4",
   pages = "601"
}

@ARTICLE{Maeno99,
    author = "Y. Maeno and S. Nakatsuji and S. Ikeda",
    year = "1999",
    journal = "Mat. Science and Engineering",
    volume = "B63",
    pages = "70"
}

@ARTICLE{Cox83,
    author = "P.A. Cox and R.G. Egdell and J.B. Goodenough and A. Hamnett and C.C. Naish",
    year = "1983",
    journal = "J. Phys. C",
    volume = "16",
    pages = "6221"
}

@ARTICLE{Cao98,
   author = "G. Cao and J. Bolivar and S. McCall and J. E. Crow and R. P. Guertin",
   year = "1998",
   journal = "Phys. Rev. B",
   volume = "57",
   pages = "R11039"
}

@ARTICLE{Mandrus99,
   author = "D. Mandrus and V. Keppens and B. C. Chakoumakos",
   year = "1999",
   journal = "Mat. Res. Bull.",
   volume = "34",
   pages = "1013"
}

@ARTICLE{Longo71,
   author = "J. M. Longo and J. A. Kafalas and R. J. Arnott",
   year = "1971",
   journal = "J. Solid State Chem.",
   volume = "3",
   pages = "174"
}

@ARTICLE{Maeno94,
   author = "Y. Maeno and H. Hashimoto and K. Yoshida and S. Nishizaki and T. Fujita and J. G. Bednorz and F. Lichtenberg",
   year = "1994",
   journal = "Nature",
   volume = "372",
   pages = "532"
}

@ARTICLE{Bernhard99,
   author = "C. Bernhard and J. L. Tallon and Ch. Niedermayer and Th. Blasius and A. Golnik and E. Br{\"u}cher and R. K. Kremer and D. R. Noakes and C. E. Stronach and E. J. Ansaldo",
   year = "1999",
   journal = "Phys. Rev. B",
   volume = "59",
   pages = "14099"
}

@ARTICLE{Sleight74,
   author = "A. W. Sleight and J. L. Gillson and J. F. Weiher and W. Bindloss",
   year = "1974",
   journal = "Solid State Comm.",
   volume = "14",
   pages = "357"
}

@ARTICLE{Slater51,
   author = "J. C. Slater",
   year = "1951",
   journal = "Phys. Rev.",
   volume = "82",
   pages = "538"
}

@INPROCEEDINGS{Matsubara54,
   author = "T. Matsubara and Y. Yokota",
   title = "Band Theory of Antiferromagnetism",
   booktitle = "Proc. Int. Conf. Theor. Phys., Kyoto-Tokyo 1953",
   year = "1954",
   publisher = "Sci. Council Japan",
   address = "Tokyo",
   pages = "693"
}

@ARTICLE{DesCloizeaux59,
   author = "J. {Des Cloizeaux}",
   year = "1959",
   journal = "J. Phys. Radium, Paris",
   volume = "20",
   pages = "606"
}

@BOOK{Mott90,
    author = "N. F. Mott",
    title = "Metal-Insulator Transitions",
    publisher = "Taylor and Francis",
    year = "1990",
    address = "London"
}

@BOOK{Fazekas99,
    author = "P. Fazekas",
    title = "Lecture Notes on Electron Correlation and Magnetism",
    publisher = "World Scientific",
    year = "1999",
    address = "Singapore"
}

@ARTICLE{Imada98,
    author = "M. Imada and A. Fujimori and Y. Tokura",
    year = "1998",
    journal = "Rev. Mod. Phys.",
    volume = "70",
    pages = "1039"
}

@ARTICLE{Subramanian83,
    author = "M. A. Subramanian and G. Aravamudan and G. V. Subba Rao",
    year = "1983",
    journal = "Prog. Solid State Chem.",
    volume = "15",
    pages = "55"
}

@ARTICLE{Donohue65,
    author = "P. C. Donohue and J. M. Longo and R. D. Rosenstein and L. Katz",
    year = "1965",
    journal = "Inorg. Chem.",
    volume = "4",
    pages = "1152"
}

@ARTICLE{Wang98,
    author = "R. Wang and A. W. Sleight",
    year = "1998",
    journal = "Mat. Res. Bull.",
    volume = "33",
    pages = "1005"
}

@ARTICLE{Sleight76,
    author = "A. W. Sleight and J. D. Bierlein",
    year = "1976",
    journal = "Solid State Comm.",
    volume = "18",
    pages = "163"
}

@ARTICLE{Allen96,
    author = "P. B. Allen and H. Berger and O. Chauvet and L. Forro and T. Jarlborg and A. Junod and
    B. Revaz and G. Santi",
    year = "1996",
    journal = "Phys. Rev. B.",
    volume = "53",
    pages = "4393"
}

@ARTICLE{Ramirez94,
    author = "A. P. Ramirez",
    year = "1994",
    journal = "Ann. Rev. Mater. Sci.",
    volume = "24",
    pages = "453"
}

@ARTICLE{Gruner94,
    author = "G. Gr{\"u}ner",
    year = "1994",
    journal = "Rev. Mod. Physics",
    volume = "66",
    pages = "1"
}

@ARTICLE{Blacklock79,
    author = "K. Blacklock and H. W. White",
    year = "1979",
    journal = "J. Chem. Phys.",
    volume = "71",
    pages = "5287"
}

@ARTICLE{Anderson56,
    author = "P. W. Anderson",
    year = "1956",
    journal = "Phys. Rev.",
    volume = "102",
    pages = "1008"
}

@ARTICLE{Pike77,
    author = "G. E. Pike and C. H. Seager",
    year = "1977",
    journal = "J. Appl. Phys.",
    volume = "48",
    pages = "5152"
}

@ARTICLE{Klein96,
    author = "L. Klein and J. S. Dodge and C. H. Ahn and G. J. Snyder and T. H. Geballe and M. R.
    Beasley and A. Kapitulnik",
    year = "1996",
    journal = "Phys. Rev. Lett.",
    volume = "77",
    pages = "2774"
}

@ARTICLE{Sullow98,
    author =  "S. Sullow and I. Prasad and M. C. Aronson and J. L. Sarrao and Z. Fisk and D. Hristova and
    A.H. Lacerda and M. F. Hundley and A. Vigliante and D. Gibbs",
    year = "1998",
    journal = "Phys. Rev. B",
    volume = "77",
    pages = "5860"
}

@ARTICLE{McCauley73,
    author = "R. A. McCauley",
    year = "1973",
    journal = "J. Opt. Soc. Amer.",
    volume = "63",
    pages = "721"
}

@ARTICLE{Reimers91,
    author = "J. N. Reimers and A. J. Berlinsky and A.-C. Shi",
    year = "1991",
    journal = "Phys. Rev. B",
    volume = "43",
    pages = "865"
}

@INCOLLECTION{Arrott66,
    author = "A. Arrott",
    title = "Antiferromagnetism in Metals",
    booktitle = "Magnetism",
    publisher = "Academic Press",
    year = "1966",
    editor = "G. T. Rado and H. Suhl",
    volume = "IIB",
    address = "New York"
}

@BOOK{Tsuda91,
    author = "N. Tsuda and K. Nasu and A. Yanase and K. Siratori",
    title = "Electronic Conduction in Oxides",
    publisher = "Springer-Verlag",
    year = "1991",
    address = "Berlin"
}

@INCOLLECTION{Chaikin90,
    author = "P. M. Chaikin",
    title = "An Introduction to Thermopower for Those who Might Want to Use it toStudy Organic
    Conductors and Superconductors",
    booktitle = "Organic Superconductivity",
    publisher = "Plenum Press",
    year = "1990",
    editor = "V. Z. Krezin and W. A. Little",
    address = "New York"
}

@ARTICLE{Sales97,
    author = "B. C. Sales and D. Mandrus and B. C. Chakoumakos and V. Keppens and J. R. Thompson",
    year = "1997",
    journal = "Phys. Rev. B",
    volume = "56",
    pages = "15081"
}

@ARTICLE{Schultz95,
    author = "W. W. Schultz and P. B. Allen",
    year = "1995",
    journal = "Phys. Rev. B",
    volume = "56",
    pages = "7994"
}

@ARTICLE{Carter91,
    author = "S. A. Carter and J. Yang and T. F. Rosenbaum and J. Spalek and J. M. Honig",
    year = "1991",
    journal = "Phys. Rev. B",
    volume = "43",
    pages = "607"
}

@ARTICLE{V2O3carter,
    author = "S. A. Carter and T. F. Rosenbaum and M. Lu and H. M. Jaeger and P. Metcalf and J. M.
    Honig and J. Spalek",
    year = "1994",
    journal = "Phys. Rev. B",
    volume = "49",
    pages = "7898"
}

@ARTICLE{blaha,
    author = "P. Blaha and K. Schwarz and P. Sorantin and S. B. Trickey",
    year = "1990",
    journal = "Comput. Phys. Commun.",
    volume = "49",
    pages = "399"
}

@ARTICLE{perdew,
    author = "J. P. Perdew and S. Burke and and M. Ernzerhof",
    year = "1996",
    journal = "Phys. Rev. Lett.",
    volume = "77",
    pages = "3865"
}

@ARTICLE{singh,
    author = "D. J. Singh",
    year = "1997",
    journal = "Phys. Rev. B",
    volume = "77",
    pages = "3865"
}

@ARTICLE{Chako84,
    author = "B. C. Chakoumakos",
    year = "1984",
    journal = "J. Solid State Chem",
    volume = "53",
    pages = "120"
}

@ARTICLE{Lynn2000,
    author = "J. W. Lynn and B. Keimer and C. Ulrich and C. Bernhard and J. L. Tallon",
    year = "2000",
    journal = "Phys. Rev. B",
    volume = "61",
    pages = "R14964"
}

